Evaluating the Efficiency of Regulation in Matching Markets with Distributional Disparities

Cap-based regulations are widely used to address distributional disparities in matching markets, but their efficiency relative to alternative instruments such as subsidies remains poorly understood. This paper develops a framework for evaluating policy interventions by incorporating regional constraints into a transferable utility matching model. We show that a policymaker with aggregate-level match data can implement a taxation policy that maximizes social welfare and outperforms any cap-based policy. Using newly collected data from the Japan Residency Matching Program, we estimate participant preferences and simulate counterfactual match outcomes under both cap-based and subsidy-based policies. The results reveal that the status quo cap-based regulation generates substantial efficiency losses, whereas small, targeted subsidies can achieve similar distributional goals with significantly higher social welfare.

==> preamble.tex <==
% Page layout
\usepackage[truedimen,margin=1in]{geometry}
\usepackage{fullpage}
\linespread{1.4}

% Language and hyphenation
\usepackage[british]{babel}
\RequirePackage[english=usenglishmax]{hyphsubst}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{textcomp}

% Color and graphics
\usepackage[dvipsnames,table,xcdraw]{xcolor}
\usepackage{graphicx}
\graphicspath{ {image/} }
\usepackage{tikz}
\usepackage{pgfplots}
%\usepackage{subfigure}
\usepackage{subcaption}

% Table formatting
\usepackage{multirow}
\usepackage{booktabs} % For formal tables
\usepackage{makecell}
\usepackage{tabularx}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}

% Algorithm and code
\usepackage[ruled]{algorithm2e}

% Math packages
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{bbm}
\usepackage{amsfonts}
\usepackage{bm}
\usepackage{mathtools} % coloneqq
\usepackage{kbordermatrix}

% Hyperlinks
\usepackage[hidelinks,hypertexnames=false,unicode]{hyperref}
\usepackage{cleveref}

% Equation numbers appear only when they are referred to
\usepackage{autonum}
%\mathtoolsset{showonlyrefs,showmanualtags} % equation numbers appear only for those used

% Document utilities
\usepackage{comment}
\usepackage{float}
\usepackage{here}
\usepackage{placeins} 
\usepackage{adjustbox}
\usepackage[toc]{appendix}
\usepackage{scalefnt}
\usepackage{setspace}
\usepackage{lipsum}
\usepackage{url}
\usepackage[flushleft]{threeparttable}
\usepackage{threeparttablex}
\usepackage{xpatch}
\usepackage[at]{easylist}

% Caption setup
\usepackage{caption}
\captionsetup[table]{labelsep=period}
\captionsetup[figure]{labelsep=period}

% Rotating content
\usepackage[figuresright]{rotating}
\usepackage{lscape}

% Bibliography
\usepackage{natbib}
\setcitestyle{authoryear}



% Theorem setup
% Define a new theorem style for upright (non-italic) body
\newtheoremstyle{myremarksandexamples}% name
    {\topsep}%      Space above
    {\topsep}%      Space below
    {}%             Body font (empty means normal upright font)
    {}%             Indent amount (empty = no indent, \parindent = indent)
    {\bfseries}%    Theorem head font (e.g., "Remark", "Example")
    {.}%            Punctuation after theorem head
    {.5em}%         Space after theorem head
    {}%             Theorem head spec (can be left empty, meaning `normal')

% Apply the default italic style to the environments that should be italic (like theorems, lemmas)
\theoremstyle{plain} % This is often the default, but good to be explicit
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{ass}{Assumption}
\newtheorem{definition}{Definition}
\newtheorem{obs}{Observation}

% Apply the new upright style for remarks and examples
\theoremstyle{myremarksandexamples}
\newtheorem{rem}{Remark}
\newtheorem{example}{Example}




% Title and sections
\usepackage{titlesec}
\usepackage{etoolbox,chngcntr}
\AtBeginEnvironment{appendices}{%
 \titleformat{\section}{\bfseries\Large}{\appendixname~\thesection:}{0.5em}{}%
 \titleformat{\subsection}{\bfseries\large}{\thesubsection}{0.5em}{}%
\counterwithin{equation}{section}
}

% Custom commands
\usepackage{dsfont}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\1}{\textbf{1}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\back}{\text{\textbackslash}}
\newcommand{\argmax}{\mathop{\rm arg~max}\limits}
\newcommand{\argmin}{\mathop{\rm arg~min}\limits}
\newcommand{\st}{\ \text{s.t.} \ }
\newcommand{\uo}{\underline{o}}
\newcommand{\bo}{\bar{o}}
\newcommand{\uw}{\underline{w}}
\newcommand{\bw}{\bar{w}}
\newcommand{\ulam}{\underline{\lambda}}
\newcommand{\blam}{\bar{\lambda}}
\newcommand{\ind}[1]{{\1\left\{ {#1} \right\}}}
\newcommand{\grad}{\nabla}
\newcommand{\prob}{\mathrm{Pr}}
\renewcommand{\epsilon}{\varepsilon}

% Optimization problem environment
\newcounter{optproblem}[section]
\makeatletter
\newenvironment{optproblem}[1]%
{%
    \protected@edef\@currentlabelname{#1}%
    \par\noindent%\vspace{\baselineskip}
    \ifx#1\empty %
    \else \refstepcounter{optproblem}$($#1$)$ %
    \fi%
    \hfill%
    $\left|%
    \hfill%
    \hspace{0.00\textwidth}%
    \@fleqntrue\@mathmargin\parindent%
    \begin{minipage}{0.86\textwidth}%
    \vspace{-0.25\baselineskip}%
}%
{%
    \vspace{-1.0\baselineskip}%
    \end{minipage}%
    \@fleqnfalse%
    \right.$%
    \par\vspace{0.5\baselineskip}\noindent%
    \ignorespacesafterend%
}%
\makeatother
\newcommand{\optprobref}[1]{$($\nameref{#1}$)$}

\newenvironment{optproblem*}%
{%
    \begin{optproblem}{}%
}%
{%
    \end{optproblem}%
    \ignorespacesafterend%
}

% Algorithm setup
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}

% Date formatting
\usepackage{datetime}
\newdateformat{monthdayyear}{\monthname[\THEMONTH] \THEDAY, \THEYEAR}
\date{\monthdayyear\today}

% comment
\newcommand{\ocomment}[1]{{\textcolor{red}{#1}}}
